Gravitation: from Newton to Einstein

This document gathers the notes of a 30-hour review course on gravitation, which I delivered in January 2018 and January 2019 at the African Institute for Mathematical Sciences of Cameroon (AIMS-Cameroon). Its main goal is to propose a big picture of gravitation, where Einstein's relativity arises as a natural increment to Newton's theory. It is designed for bachelor/master students who do not necessarily have prior knowledge about relativity. The students are nevertheless expected to be familiar with the fundamentals of Newton's mechanics and gravitation, for the first chapter to be a mere reformulation of known concepts. The second chapter then introduces special and general relativity at the same time, while the third chapter explores concrete manifestations of relativistic gravitation, notably gravitational waves and black holes. Each section corresponds, on average, to slightly more than a 2-hour black-board lecture. The numerous exercises must be considered part of the course itself; they are intended to stimulate active reading.

==> style.tex <==
\geometry{a4paper,top=2.5cm,headheight=1.7cm,headsep=1cm,bottom=2.5cm,inner=2.5cm,outer=2.5cm}

% This forces the page potentially introduced with \cleardoublepage to be white
\makeatletter
\renewcommand{\cleardoublepage}{%
  \clearpage\thispagestyle{empty}%
  \if@twoside
    \ifodd\c@page
      %
    \else
      \hbox{}\newpage
      \if@twocolumn
         \hbox{}\newpage
      \fi
    \fi
  \fi}
\makeatother

\makeatletter
\newcommand*{\cleartoleftpage}{%
  \clearpage
    \if@twoside
    \ifodd\c@page
      \hbox{}\newpage
      \if@twocolumn
        \hbox{}\newpage
      \fi
    \fi
  \fi
}
\makeatother


% New style for chapters and sections, using package titlesec

\newlength{\chapterrulelength}
\newlength{\chapterlabellength}
\newcommand{\mychapterlabel}{\colorbox{black}{\color{white}\huge\textsc{\chaptertitlename}~\thechapter}}

\renewcommand{\thechapter}{\Roman{chapter}}
\titleformat{\chapter}
[display]%shape
  {}%format
  {\settowidth{\chapterlabellength}{\mychapterlabel}
  \setlength{\chapterrulelength}{\textwidth}
  \addtolength{\chapterrulelength}{-\chapterlabellength}
  \rule[-3pt]{\chapterrulelength}{2pt}\mychapterlabel}%label
  {8pt}%sep
  {\sffamily\bfseries\Huge}%before code
  %[]after code
  
\renewcommand{\thesection}{\Roman{chapter}.\Alph{section}}
%\renewcommand{\thesubsection}{\arabic{subsection}}
\titlelabel{\thetitle.\quad}

\titleformat{\paragraph}[runin]{\sf\bfseries}{}{}{%
%\textcolor{mygray}{
$\blacksquare$
%}
\hspace{0.1cm}}

% Page style

\newlength{\pageboxlength}
\settowidth{\pageboxlength}{000}
\newlength{\cornerdrag}
\setlength{\cornerdrag}{0.5cm}
\addtolength{\cornerdrag}{\pageboxlength}

\fancypagestyle{plain}{%
\fancyhf{}
\fancyhead[LE]{\hspace*{-\cornerdrag}\makebox[\pageboxlength][r]{\sf\thepage}}
\fancyhead[RO]{\makebox[\pageboxlength][l]{\sf\thepage}\hspace*{-\cornerdrag}}
}

\pagestyle{fancy}
\fancyhf{}
\renewcommand{\sectionmark}[1]{\markright{\thesection \: #1}}
\renewcommand{\chaptermark}[1]{\markboth{\chaptername \ \thechapter \quad #1}{}}
\renewcommand{\headrulewidth}{0pt}
\fancyhead[LE]{\hspace*{-\cornerdrag}\makebox[\pageboxlength][r]{\sf\thepage}\hspace{0.5cm}\rule{1pt}{1.5cm}\hspace{0.5cm}\nouppercase{\sf\slshape\leftmark}}
\fancyhead[RE]{}
\fancyhead[LO]{}
\fancyhead[RO]{\nouppercase{\sf\slshape\rightmark}\hspace{0.5cm}\rule{1pt}{1.5cm}\hspace{0.5cm}\makebox[\pageboxlength][l]{\sf\thepage}\hspace*{-\cornerdrag}}
\cfoot{}
